Reconstructing Video from Interferometric Measurements of Time-Varying Sources

Very long baseline interferometry (VLBI) makes it possible to recover images of astronomical sources with extremely high angular resolution. Most recently, the Event Horizon Telescope (EHT) has extended VLBI to short millimeter wavelengths with a goal of achieving angular resolution sufficient for imaging the event horizons of nearby supermassive black holes. VLBI provides measurements related to the underlying source image through a sparse set spatial frequencies. An image can then be recovered from these measurements by making assumptions about the underlying image. One of the most important assumptions made by conventional imaging methods is that over the course of a night's observation the image is static. However, for quickly evolving sources, such as the galactic center's supermassive black hole (Sgr A*) targeted by the EHT, this assumption is violated and these conventional imaging approaches fail. In this work we propose a new way to model VLBI measurements that allows us to recover both the appearance and dynamics of an evolving source by reconstructing a video rather than a static image. By modeling VLBI measurements using a Gaussian Markov Model, we are able to propagate information across observations in time to reconstruct a video, while simultaneously learning about the dynamics of the source's emission region. We demonstrate our proposed Expectation-Maximization (EM) algorithm, StarWarps, on realistic synthetic observations of black holes, and show how it substantially improves results compared to conventional imaging algorithms. Additionally, we demonstrate StarWarps on real VLBI data of the M87 Jet from the VLBA.

==> paperparts/figures/compare_1.tex <==
\begin{figure*}
	\begin{center}
		\vspace{-0.5in}
		%\hspace*{-2.3cm}
		\setlength{\tabcolsep}{3pt}
		
		\hspace{-0.8in}\normalsize{\textsf{BLURRED TRUE MEAN}}  \hspace{4.5cm} \normalsize{\textsf{NORMALIZED RMSE}} 
		\vspace{0.1in}
		
		
%	\begin{tabular}{ c " c}
%		VIDEO 1& VIDEO 2 \\ \thickhline
%		& \vspace{-.1in} \\
%		VIDEO 3 & VIDEO 4
%	\end{tabular}
%	\qquad
%		\begin{tabular}{ c " c}
%		{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_15_blurredbeam75_noaxis.pdf}} } & {{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_115_blurredbeam75_noaxis.pdf}} } \\ \thickhline
%		& \vspace{-.1in} \\
%	{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/gt/frames/gt_85_blurredbeam75_noaxis.pdf}} } & {{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/gt/frames/gt_63_blurredbeam75_noaxis.pdf}} }
%		\end{tabular}
						\begin{tabular}{ c " c}
							{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/gt/pavgImg_blurredbeam75_noaxis.pdf}} } & {{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/gt/pavgImg_blurredbeam75_noaxis.pdf}} } \\ \thickhline
							& \vspace{-.1in} \\
							{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/gt/pavgImg_blurredbeam75_noaxis.pdf}} } & {{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/gt/pavgImg_blurredbeam75_noaxis.pdf}} }
						\end{tabular}	
	%	\qquad	
		\qquad
		\begin{tabular}{ r | c | c | c | c " c | c | c | c}
			& \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017}} } \rotatebox[origin=t]{90}{\small{\textsf{VIS}} }  & \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} } & \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017+}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} } &\rotatebox[origin=t]{90}{\small{\textsf{FUTURE}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} } & \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017}} } \rotatebox[origin=t]{90}{\small{\textsf{VIS}} }  & \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} } & \rotatebox[origin=t]{90}{\small{\textsf{EHT 2017+}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} } &\rotatebox[origin=t]{90}{\small{\textsf{FUTURE}} } \rotatebox[origin=t]{90}{\small{\textsf{AMP \& BISP}} }  \\ \hline
			\small{\textsf{StarWarps} & \bm{0.67} & \bm{0.65}& \bm{0.55}&  \bm{0.55}& \bm{0.74} & \bm{0.73} & \bm{0.73} &  0.71 \\ 
			\cite{freek} & 1.05  & 0.82 & 0.73  & 0.68 &  0.98 & 1.21 & 0.99 & 0.35 \\ 
			\cite{andrew} & 0.79 & 0.80 & 0.73 & 0.63 & 0.83& 1.05 & 0.81 & \bm{0.23}  \\  \thickhline
			StarWarps & \bm{0.32} & \bm{0.55} & 0.67 & \bm{0.36} & \bm{0.34} & \bm{0.44} & \bm{0.23} & \bm{0.31} \\
			\cite{freek} & 0.93 & 0.90 & \bm{0.53} & 0.51 & 0.84 & 0.75 & 1.02 & 0.61 \\
			\cite{andrew} &0.84 & 0.85 & 0.71 &  0.39  & 0.60 & 0.50 & 0.60 & 0.47
		\end{tabular}

		\vspace{0.2in}
		
		\hspace*{-1.3cm}
		\begin{tabular}{  c c | c  c  c  c "  c  c  c  c  }
			%\hline
			& \large{\textsf{Array:}} &\small{\textsf{EHT 2017}}   &\small{\textsf{EHT 2017 }} &\small{\textsf{EHT2017+}}    &\small{\textsf{FUTURE}}    &\small{\textsf{EHT 2017}}   &\small{\textsf{EHT 2017 }} &\small{\textsf{EHT2017+}}    &\small{\textsf{FUTURE}}     \\ 
			&\vspace{-.1in} & & & & & & & &\\
			& \large{\textsf{Data:}} &\small{\textsf{VIS}}   &\small{\textsf{AMP \& BISP}} &\small{\textsf{AMP \& BISP}}    &\small{\textsf{AMP \& BISP}}  &\small{\textsf{VIS}}   &\small{\textsf{AMP \& BISP}} &\small{\textsf{AMP \& BISP}}    &\small{\textsf{AMP \& BISP}}   \\ \hline
			&\vspace{-.1in} & & & & & & & &\\
			\multirow{2}{*}[0.2in]{ \rotatebox[origin=t]{90}{\small{\textsf{StarWarps}} }}   \hspace{-0.3in} & \multirow{1}{*}[0.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{FRAME}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_visibility/nomotion/frames/mean_noaxis_15.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_amp-bispectrum/nomotion/frames/mean_noaxis_15.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_15.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture1_100_amp-bispectrum/nomotion/frames/mean_noaxis_15.pdf}  
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_visibility/nomotion/frames/mean_noaxis_115.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_amp-bispectrum/nomotion/frames/mean_noaxis_115.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_115.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture1_100_amp-bispectrum/nomotion/frames/mean_noaxis_115.pdf} \\
			&\vspace{-.1in} & & & & & & & &\\
			&	\multirow{1}{*}[0.6in]{ \rotatebox[origin=t]{90}{\small{\textsf{MEAN}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_visibility/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture1_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_visibility/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture1_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} 
			\\   \hline
			&\vspace{-.1in} & & & & & & & &\\
			\multirow{2}{*}[0.6in]{ \rotatebox[origin=t]{90}{\small{\textsf{MEM \& TV Regularization}} }}  \hspace{-0.3in} & \multirow{1}{*}[0.4in]{ \rotatebox[origin=t]{90}{\small{\textsf{\cite{freek}}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_vis_rotation30_tint100_eht2017_directim_maxit100_it0.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_rotation30_tint100_eht2017_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_rotation30_tint100_ehtfuture2_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_rotation30_tint100_ehtfuture1_directim_maxit100_it0.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_vis_hotspot100sR2_tint100_eht2017_directim_maxit100_it0.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotspot100sR2_tint100_eht2017_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotspot100sR2_tint100_ehtfuture2_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotspot100sR2_tint100_ehtfuture1_directim_maxit100_it0.pdf} 
			\\
			&\vspace{-.1in} & & & & & & & &\\
			&	\multirow{1}{*}[0.4in]{ \rotatebox[origin=t]{90}{\small{\textsf{\cite{andrew}}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_compare/none_vis_blur025.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/eht2017_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture2_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/rotation30/ehtfuture1_100_compare/none_amp-clphase_blur025.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_compare/none_vis_blur025.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/eht2017_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture1_100_compare/none_amp-clphase_blur025.pdf} 
			\\   \thickhline
			
			&\vspace{-.1in} & & & & & & & &\\
			\multirow{2}{*}[0.2in]{ \rotatebox[origin=t]{90}{\small{\textsf{StarWarps}} }}  \hspace{-0.3in} & \multirow{1}{*}[0.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{FRAME}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_visibility/nomotion/frames/mean_noaxis_85.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_amp-bispectrum/nomotion/frames/mean_noaxis_85.pdf} 
			%\includegraphics[height=.1\linewidth]{figures/starwarps_results/starwarps_hotaka02_2/nomotion/mean_85.png} 
			&
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_85.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture1_100_amp-bispectrum/nomotion/frames/mean_noaxis_85.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_visibility/nomotion/frames/mean_noaxis_63.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_amp-bispectrum/nomotion/frames/mean_noaxis_63.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_63.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture1_100_amp-bispectrum/nomotion/frames/mean_noaxis_63.pdf} \\
			&\vspace{-.1in} & & & & & & & &\\
			&	\multirow{1}{*}[0.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{MEAN}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_visibility/nomotion/pavgimg_noaxis.pdf}} } 
			&
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} 
			%\includegraphics[height=.1\linewidth]{figures/starwarps_results/starwarps_hotaka02_2/avgImg.pdf} 
			&
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture1_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_visibility/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture1_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf} 
			\\   \hline
			&\vspace{-.1in} & & & & & & & &\\
			\multirow{2}{*}[0.6in]{ \rotatebox[origin=t]{90}{\small{\textsf{MEM \& TV Regularization}} }}  \hspace{-0.3in} & 	\multirow{1}{*}[0.4in]{ \rotatebox[origin=t]{90}{\small{\textsf{\cite{freek}}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_vis_hotakamovie_02_16300_20999_tint100_eht2017_directim_maxit100_it0.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_02_16300_20999_tint100_eht2017_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_02_16300_20999_tint100_ehtfuture2_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_02_16300_20999_tint100_ehtfuture1_directim_maxit100_it0.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_vis_hotakamovie_45_16300_20999_tint100_eht2017_directim_maxit100_it0.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_45_16300_20999_tint100_eht2017_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_45_16300_20999_tint100_ehtfuture2_directim_maxit100_it0.pdf} &
			\includegraphics[height=.1\linewidth]{figures/freeksmoothingresults/im_apar_hotakamovie_45_16300_20999_tint100_ehtfuture1_directim_maxit100_it0.pdf} 
			\\
			&\vspace{-.1in} & & & & & & & &\\
			&	\multirow{1}{*}[0.4in]{ \rotatebox[origin=t]{90}{\small{\textsf{\cite{andrew}}} }}
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_compare/none_vis_blur025.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/eht2017_100_compare/none_amp-clphase_blur025.pdf} 
			&
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture2_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_02/ehtfuture1_100_compare/none_amp-clphase_blur025.pdf} 
			&
			{{\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_compare/none_vis_blur025.pdf}} } &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/eht2017_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture2_100_compare/none_amp-clphase_blur025.pdf} &
			\includegraphics[height=.1\linewidth]{figures/starwarps_results/hotakamovie_45/ehtfuture1_100_compare/none_amp-clphase_blur025.pdf} 
			\\   \hline
		\end{tabular}
		\caption{{\bf Static evolution model:} Results obtained using data simulated from each of the 4 video sequences (see Figure~\ref{fig:groundtruth}) under different telescope arrays (see Figures~\ref{fig:staticimaging} and~\ref{fig:uvcov2}) and noise conditions. The main portion of the figure is broken up into 4 quadrants corresponding to Videos 1-4 when moving from left to right, top to bottom. The true single frame and mean image from the ground truth videos, blurred to 3/4 the nominal resolution of the array, are shown on the top. We compare results of our proposed method, StarWarps, to that of the single imaging methods presented in~\cite{freek} and~\cite{andrew}. The data type VIS indicates using visibilities on data with no atmospheric error, while the data type AMP \& BISP indicates using the visibility amplitudes and bispectrum on data where atmospheric phase errors have been introduced. }
		\label{fig:staticevolutionresults}
	\end{center}
\end{figure*}





























































==> paperparts/figures/rotation_example.tex <==
%\begin{figure*}[h!]
%\begin{center}
%	 \hspace*{-1.5cm}
%    \begin{tabular}{  c | c | c  c  c  c  c c }
%        %\hline
%        &\large{\textsf{Mean + Flow}}   &\large{\textsf{t = 1 }} &\large{\textsf{t = 7 }}    &\large{\textsf{t = 13 }} &\large{\textsf{t = 19 }}  &\large{\textsf{t = 25 }}  &\large{\textsf{t = 30 }}     \\ \hline
%
%		&\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
%        &
%		{{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_29.pdf} 
%         \\   \hline
%         %&\vspace{.0001in}& \\
%         \multicolumn{8}{c}{  \large{\textsf{EHT 2017 WITH CALIBRATED DATA}}  }
%         \\ \hline
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{No Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_29.pdf} 
%        \\          
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_29.pdf}  
%		 \\ \hline  	
%		 %&\vspace{.0001in}& \\
%		 \multicolumn{8}{c}{  \large{\textsf{EHT 2017+ WITH UNCALIBRATED DATA }}  }
%		\\ \hline
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{No Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_29.pdf} 
%        \\          
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 1}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_29.pdf}  
%        \\ 
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 2}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_29.pdf}  
%        \\ \hline  	
%    \end{tabular}
%    \caption{\footnotesize{  }}
%\label{fig:rotation_example}
%\end{center}
%\end{figure*}







\begin{figure*}
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		%\hspace*{-1.5cm}
		\begin{tabular}{  c | c | c  c  c  c  c c }
			
			
			%\hline
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{\large{\textsf{uv-coverage}} }} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/uv_ehtfuture2_rotation30_small.pdf} 
			&
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_29.pdf} 
			\\  \hline
			&\vspace{-.1in} &&&&&&\\ 
			
			
			&\large{\textsf{Mean Frame}}   &\large{\textsf{GST = 17:00}} &\large{\textsf{19:30}}    &\large{\textsf{22:00}} &\large{\textsf{00:30}}  &\large{\textsf{03:00}}  &\large{\textsf{05:30}}     \\ \hline
			
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_29.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH CALIBRATED DATA (VIS) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Average_Snapshot_vis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/flow_pavg_best_noaxiscrop.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_29.pdf}  
			\\ \hline  	
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH ATMOSPHERIC PHASE ERROR (AMP \& BISP) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Average_Snapshot_AmpCphase.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/flow_pavg_best_noaxiscrop.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_29.pdf}  
			%			\\ 
			%			&\vspace{-.1in} &&&&&&\\
			%			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 2}} }}
			%			&
			%			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/flow_pavg_best.pdf}} } &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_0.pdf} &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_6.pdf} &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_12.pdf} &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_18.pdf} &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_24.pdf} &
			%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_29.pdf}  
			\\ \hline  	
		\end{tabular}
		\caption{{\bf Time-resolved reconstruction of Video 1:} Video 1 contains an image rotating clockwise by $180^{\circ}$ over the course of the observation. At each time, the interferometric telescope array measures values related to 2D spatial frequencies of the current underlying image, shown in the row labeled `Truth'. These are indicated by the dots on the uv-coverage plots. As light emitted from the source is real-valued we obtain two values on opposite sides of the frequency plane -- each independent set of measurements displayed as either black or red. We present results obtained when using data with no atmospheric error (VIS) as well as when there is atmospheric phase error and we must use data products invariant to its effects (AMP \& BISP).
			Below the true images, we show a subset of images from the baseline 'snapshot imaging' method and compare it to our StarWarps reconstructed video obtained when we assume a static warp field or an inferred warp field. The mean image for each sequence is shown in the leftmost column. In the case that we simultaneously estimate a warp field, we indicate the resulting field as arrows on the mean image. Our method substantially improves results over the snapshot method, especially in the case of atmospheric error when the absolute position of the source cannot be recovered. Additionally, our proposed method can estimate a warp field that gives a sense of the underlying motion of the emission region. This can help to improve results, most notably for the calibrated data (VIS). }
		\label{fig:rotation_example1}
	\end{center}
\end{figure*}





















\begin{figure*}
	\begin{center}
		\setlength{\tabcolsep}{1pt}
		%\hspace*{-1.5cm}
		\begin{tabular}{  c | c | c  c  c  c  c c }
			%\hline
			
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{\large{\textsf{uv-coverage}} }}
			&
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/uv_ehtfuture2_small.pdf} 
			&
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSf.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			
			&\large{\textsf{Mean Frame}}   &\large{\textsf{GST = 20:10 }} &\large{\textsf{20:20 }}    &\large{\textsf{20:30 }} &\large{\textsf{20:40 }}  &\large{\textsf{20:50 }}  &\large{\textsf{21:00 }}     \\ \hline
			
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSf.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH CALIBRATED DATA (VIS) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Average_Snapshot_vis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/flow_pavg_best_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSf.pdf} 
			\\ \hline  	
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH ATMOSPHERIC PHASE ERROR (AMP \& BISP) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Average_Snapshot_AmpCphase.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSf.pdf}  \\
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/flow_pavg_best_noaxis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_49.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_59.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_69.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_79.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_89.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_90.pdf}  
			\\ \hline  	
		\end{tabular}
		\caption{{\bf Time-resolved reconstruction of Video 2:} Video 2 contains a sequence of a hotspot orbiting counter-clockwise around a black hole. We present time-resolved results obtained using data derived from this sequence. 
			Below the true images, we show a subset of images from the baseline 'snapshot imaging' method and compare it to our StarWarps reconstructed video obtained assuming a static warp field or an inferred warp field. The mean image for each sequence is shown in the leftmost column. If we simultaneously estimate a warp field, we indicate the resulting field as arrows on the mean image. 
			Our method substantially improve results over the snapshot method, especially in the case of atmospheric error when the absolute position of the source cannot be recovered. 
			Additionally, despite the fact that this hotspot video does not match our assumed motion model, using our proposed approach we were able to estimate a warp field that provides the direction of the source's true underlying motion. See the caption of Figure~\ref{fig:rotation_example1} for more detail. }
		\label{fig:rotation_example2}
	\end{center}
\end{figure*}




==> paperparts/figures/singleimage_old.tex <==
\begin{figure*}[h!]
	
	\begin{center}
		\begin{tabular}{ c  c  c  c   }
			%\hline
			\hspace*{-1.5cm} \multirow{4}{*}[-0in]{ \rotatebox[origin=t]{0}{ {\vspace{10in} \includegraphics[height=.35\linewidth]{figures/uvcoverage/uv_eht2017.pdf}}
					\qquad  }} &  \hspace{-1cm} \large{\textsf{True Static Image}}   &\large{\textsf{MEM \& TV Recon.}} &\large{\textsf{CHIRP Recon.}}      \\
			&\hspace{-1cm} {{\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe.pdf}} } &
			{\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe_andrew.pdf}} &
			{\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe_chirp.pdf}} 
			\\
			& \vspace{-.1in}
			\\
			& \hspace{-1cm} \large{\textsf{Gauss Recon.}}   &\large{\textsf{Clipped Gauss Recon.}} &\large{\textsf{Estimated SNR} }     \\
			&\hspace{-1cm} {{\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe_gauss.pdf}} } &
			\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe_gaussnneg.pdf} &
			\includegraphics[height=.16\linewidth]{figures/singleimage/hotakaframe_gausssnr.pdf} 
			\\
		\end{tabular}
		\caption{{\bf Static Imaging Comparison:} Results of static imaging using a multivariate Gaussian prior (a=2) compared to state-of-the-art reconstruction methods using MEM \& TV regularizers~\cite{andrew} as well as patch-based regularizers (CHIRP)~\cite{bouman2016computational}. Data is generated using a static image with the uv-coverage of the EHT2017 array shown on the left (see Section~\ref{sec:results}). The uv-coverage is colored by time, as indicated by the colorbar in Figure~\ref{fig:uvcov2} \michael{I'm not sure the journal will let you forward reference a figure.}. In addition to realistic thermal noise, atmospheric phase errors have been included in the data. Although the previous algorithms (MEM \& TV and CHIRP) both produce better results, the Gaussian reconstruction is able to correctly get the broad structure of the underlying image. Since we do not impose positivity, negative values are reconstructed. However, by clipping the resulting image we can see that the result aligns well with the true static image. The Gaussian prior model also allows us to easily estimate the SNR of our reconstruction using the diagonal entries of the posterior covariance matrix. \michael{I don't understand how to interpret the SNR. Also, why is it in dB? Is it a relative value among image pixels? The SNR seems to be lowest in regions of the images that are reliably reconstructed...)}} 
		\label{fig:staticimaging}
	\end{center}
\end{figure*}


==> paperparts/results_comp.tex <==


















%\begin{figure*}[h!]
%\begin{center}
%	 \hspace*{-1.5cm}
%    \begin{tabular}{  c | c | c  c  c  c  c c }
%        %\hline
%        &\large{\textsf{Mean + Flow}}   &\large{\textsf{t = 1 }} &\large{\textsf{t = 7 }}    &\large{\textsf{t = 13 }} &\large{\textsf{t = 19 }}  &\large{\textsf{t = 25 }}  &\large{\textsf{t = 30 }}     \\ \hline
%
%		&\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
%        &
%		{{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/gt/frames/gt_29.pdf} 
%         \\   \hline
%         %&\vspace{.0001in}& \\
%         \multicolumn{8}{c}{  \large{\textsf{EHT 2017 WITH CALIBRATED DATA}}  }
%         \\ \hline
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{No Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/nomotion/frames/mean_29.pdf} 
%        \\          
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/visibilities/best/frames/mean_29.pdf}  
%		 \\ \hline  	
%		 %&\vspace{.0001in}& \\
%		 \multicolumn{8}{c}{  \large{\textsf{EHT 2017+ WITH UNCALIBRATED DATA }}  }
%		\\ \hline
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{No Flow}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/pavgimg.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/nomotion/frames/mean_29.pdf} 
%        \\          
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 1}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30Jy2/amp-bispectrum/best/frames/mean_29.pdf}  
%        \\ 
%        &\vspace{-.15in}&\\
%        \multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 2}} }}
%        &
%        {{\includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/flow_pavg_best.pdf}} } &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_0.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_6.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_12.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_18.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_24.pdf} &
%        \includegraphics[height=0.1\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_29.pdf}  
%        \\ \hline  	
%    \end{tabular}
%    \caption{\footnotesize{  }}
%\label{fig:rotation_example}
%\end{center}
%\end{figure*}







\begin{figure*}[h!]
	\begin{center}
		\hspace*{-1.5cm}
		\begin{tabular}{  c | c | c  c  c  c  c c }
			%\hline
							\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{\large{\textsf{uv-coverage}} }} &
											\includegraphics[height=0.12\linewidth]{figures/uvcoverage/uv_ehtfuture2_rotation30_small.pdf} 
							&
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_0.pdf} &
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_6.pdf} &
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_12.pdf} &
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_18.pdf} &
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_24.pdf} &
							\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_30/uv_ehtfuture2_rotation30_29.pdf} 
							\\  \hline
							&\vspace{-.1in} &&&&&&\\ 
							
							
			&\large{\textsf{Mean Frame}}   &\large{\textsf{time = 00:00}} &\large{\textsf{02:30}}    &\large{\textsf{05:00}} &\large{\textsf{07:30}}  &\large{\textsf{10:00}}  &\large{\textsf{12:30}}     \\ \hline
			
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/gt/frames/gt_noaxis_29.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH CALIBRATED DATA (VIS) }}  }
			\\ \hline
				&\vspace{-.1in} &&&&&&\\
				\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
				&
				{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Average_Snapshot_vis.pdf}} } &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_0.pdf} &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_6.pdf} &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_12.pdf} &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_18.pdf} &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_24.pdf} &
				\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_vis_29.pdf} 
				\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/nomotion/frames/mean_noaxis_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/flow_pavg_best.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/visibilities/best/frames/mean_noaxis_29.pdf}  
			\\ \hline  	
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH ATMOSPHERIC PHASE ERROR (AMP \& BISP) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Average_Snapshot_AmpCphase.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/rotation30_ehtfuture2_300_snapshot/Reconstructed_Snapshot_AmpCphase_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/nomotion/frames/mean_noaxis_29.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/flow_pavg_best.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_0.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_6.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_12.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_18.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_24.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol1/best/frames/mean_noaxis_29.pdf}  
%			\\ 
%			&\vspace{-.1in} &&&&&&\\
%			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Flow 2}} }}
%			&
%			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/flow_pavg_best.pdf}} } &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_0.pdf} &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_6.pdf} &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_12.pdf} &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_18.pdf} &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_24.pdf} &
%			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/rotation30/amp-bispectrum_sol2/best/frames/mean_noaxis_29.pdf}  
			\\ \hline  	
		\end{tabular}
		\caption{{\bf Time-resolved reconstruction of Video 1:} Video 1 contains an image rotating clockwise by $180^{\circ}$ over the course of the observation. At each time, the interferometric telescope array measures values related to 2D spatial frequencies of the current underlying image, shown in the row labeled Truth. These are indicated by the dots on the uv-coverage plots. Note that as the emission we observe is real-valued we obtain two values on opposite sides of the frequency plane -- each independent set of measurements displayed as either black or red. We present results obtained when using data with no atmospheric error (VIS) as well as when there is atmospheric phase error and we must use data products invariant to its effects (AMP \& BISP).
		Below the true images, we show a subset of images from the baseline 'snapshot imaging' method and compare it to our StarWarps reconstructed video obtained when we assume a static warp field or an inferred warp field. The mean image for each sequence is shown in the leftmost column. In the case that we simultaneously estimate a warp field, we indicate the resulting field as arrows on the mean image. We find that our results substantially improve results over the snapshot method, especially in the case of atmospheric error when the absolute position of the source cannot be recovered. Additionally, our proposed method allows us to estimate a warp field that gives us a sense of the underlying motion of the emission. This can help to improve results, most notably in the results shown on calibrated data (VIS). }
		\label{fig:rotation_example1}
	\end{center}
\end{figure*}





















\begin{figure*}[h!]
	\begin{center}
		\hspace*{-1.5cm}
		\begin{tabular}{  c | c | c  c  c  c  c c }
			%\hline
			
			\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{\large{\textsf{uv-coverage}} }}
			&
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/uv_ehtfuture2_small.pdf} 
			&
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/uvcoverage/ehtfuture2_173/uv_ehtfuture2_\HSf.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			
			&\large{\textsf{Mean Frame}}   &\large{\textsf{t = \HSa }} &\large{\textsf{t = \HSb }}    &\large{\textsf{t = \HSc }} &\large{\textsf{t = \HSd }}  &\large{\textsf{t = \HSe }}  &\large{\textsf{t = \HSf }}     \\ \hline
			
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\large{\textsf{Truth}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/gt/frames/gt_noaxis_\HSf.pdf} 
			\\   \hline
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH CALIBRATED DATA (VIS) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Average_Snapshot_vis.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_vis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/nomotion/frames/mean_noaxis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
		\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/flow_pavg_best.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_visibility/best/frames/mean_noaxis_\HSf.pdf} 
			\\ \hline  	
			&\vspace{-.1in} &&&&&&\\
			\multicolumn{8}{c}{  \large{\textsf{EHT2017+ WITH ATMOSPHERIC PHASE ERROR (AMP \& BISP) }}  }
			\\ \hline
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[.5in]{ \rotatebox[origin=t]{90}{\small{\textsf{Snapshot}} }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Average_Snapshot_AmpCphase.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/hotspot100sR2_ehtfuture2_100_snapshot/Reconstructed_Snapshot_AmpCphase_\HSf.pdf}  \\
			&\vspace{-.1in} &&&&&&\\
			\multirow{1}{*}[0.7in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{No Warp}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/pavgimg.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSa.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSb.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSc.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSd.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSe.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/nomotion/frames/mean_noaxis_\HSf.pdf} 
			\\          
			&\vspace{-.1in} &&&&&&\\
\multirow{1}{*}[0.85in]{ \rotatebox[origin=t]{90}{  \specialcell{ \small{\textsf{StarWarps:}} \\  \small{\textsf{Infer Warp Field}}}  }}
			&
			{{\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/flow_pavg_best.pdf}} } &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_49.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_59.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_69.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_79.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_89.pdf} &
			\includegraphics[height=0.12\linewidth]{figures/starwarps_results/hotspot100sR2/ehtfuture2_100_amp-bispectrum/best/frames/mean_noaxis_90.pdf}  
			\\ \hline  	
		\end{tabular}
		\caption{{\bf Time-resolved reconstruction of Video 2:} Video 2 contains a sequence of a hotspot orbiting counter-clockwise around a black hole. We present time-resolved results obtained when using data derived from this sequence. 
		Below the true images, we show a subset of images from the baseline 'snapshot imaging' method and compare it to our StarWarps reconstructed video obtained when we assume a static warp field or an inferred warp field. The mean image for each sequence is shown in the leftmost column. In the case that we simultaneously estimate a warp field, we indicate the resulting field as arrows on the mean image. 
		We find that our results substantially improve results over the snapshot method, especially in the case of atmospheric error when the absolute position of the source cannot be recovered. 
		Additionally, despite the fact that this hotspot video does not perfectly match our assumed motion model, using our proposed approach we were able to estimate a warp field that gives us a sense of the true underlying motion of the emission. See the caption of Figure~\ref{fig:rotation_example1} for more detail. \katie{put the real times} }
		\label{fig:rotation_example2}
	\end{center}
\end{figure*}



==> paperparts/setup.tex <==


\section{Image and Data Models}
\label{sec:setup}

Before discussing how to reconstruct images from the data products discussed in Section~\ref{sec:meas}, it is first important to show how to generate samples of these data products from a known emission image.
%underlying image %or video 
%of the emission. 

%Constructing a generative model of the samples is important in 

\subsection{Image}

An image of instantaneous emission, $I(\xpos,\ypos)$, is defined over the continuous space of angular coordinates $\xpos$ and $\ypos$. However, to make computation tractable,
we represent this continuous image as a square $M \times M$ array of values that represent the emission image's flux over a specified field of view (FOV). 

Following the image parameterization convention of BLAH, we represent the continuous image, $I$, as the sum of a discrete number of scaled and shifted triangle pulses of height $\im$ centered around $(\xpos, \ypos) \in L \times L$, where

\begin{align}
L &=  \left \{ k \Delta + \frac{\Delta}{2}  -\frac{FOV}{2} \right \} \hspace{0.26in} \mbox{for} \hspace{0.1 in} k = 0,...,M-1
\label{eq:discrete1}
\end{align} 


\noindent{for $\Delta = \frac{FOV}{\npix}$. Using this representation, we are able to describe the 2D continuous image as a vector, $\im$, of length $M^2$. When applicable, we denote a single image in a sequence of images as $\im_t$, where $t$ indexes the time of the instantaneous image.}

%By representing $I(\xpos, \ypos)$ as its vectorized coefficients, $x$, we are able to represent a continuous image using a discrete number of terms. 

\subsection{Data Products}
\label{sec:dataproducts}

In order to evaluate how consistent a proposed image, $\im$, is with the measured VLBI data, $\meas$, we construct a function $f(\im)$ that returns the values we would expect to see in $\meas$ if $\im$ were the true underlying image, and no additional noise was added. This measurement function, $f(\im)$, is composed of a set of sub-functions, $g_k(\im)$, that each simulate an ideally observed data product: 

\begin{align}
f(\im) = \Spvek{g_1(\im); g_2(\im); ...; g_{\nmeas}(\im)} : \Re^{ M^2 \times 1} \rightarrow \Re^{ \nmeas \times 1 }
\end{align}

Each $g_k(\im)$ produces a real-value corresponding to element $k$ of the vector $\meas$. For example, $g_k(\im)$ may return the imaginary portion of $\im$'s spatial frequency, corresponding to the visibility obtained between a pair of telescopes.

Depending on the data products selected for $\meas$, the measurement function, $f(\im)$, may be a linear or non-linear function of $\im$. Although this choice does not affect the quality of the values produced by $f(\im)$, it does affect the optimization process during inference (refer to Section~\ref{sec:static}). % and~\ref{sec:dynamic_inference}). %Thus, we list the cases when the measurement function can be expressed linearly or must require a non-linear function.  
Below we list the cases when a data product can be expressed linearly or requires a non-linear function. In the supplemental material we provide the exact measurement function used for each data product and their derivatives. 

\vspace{.1in}
\subsubsection{Linear Measurement Functions}
\label{sec:dataproducts_lin}
%The question remains how to define each $g(x)$. 
Since each measured complex visibility is approximated as the Fourier transform of $I(\xpos,\ypos)$, we can extract an image's ideal visibilities by performing a linear matrix operation similar to a Discrete Time Fourier Transform (DTFT): $f(\im) = \FTmtx \im$.
%When complex visibilities can be used for image reconstruction, $f(\im)$ is expressed simply as a linear matrix operation: $f(\im) = \FTmtx \im$. 
In particular, BLAH shows that by plugging the parameterized image, $\im$, into the van Cittert-Zernike theorem (Equation~\ref{eq:vcz}), we can express a single visibility as $\im$ multiplied by a complex row-vector $\vecFTmtx(u,v)$ of size $1 \times \npix^2$.  $\FTmtx$ is then constructed by stacking the real and imaginary components of these row vectors for each of sampled $(u,v)$ point into a matrix of size $\nmeas \times \npix^2$. 
%Additionally, blurring via convolution to simulate interstellar scattering is also a linear operation and can be represented in an 


%\begin{align}
%f(\im) = \FTmtx \im = \Spvek{\Re \left[ \vecFTmtx(u,v) \right]; \Im \left[ \vecFTmtx(u,v) \right]} \im 
%\end{align}

\vspace{.1in}
\subsubsection{Non-Linear Measurement Functions}
In the case of atmospheric noise, uniformly random phase errors are included in each complex visibility measurements. 
%However, these phase errors are incorporated in a way that preserves closure phase (refer to Section BLAH). 
In order to handle this additional phase error, without having to explicitly model the errors as latent variables, we populate $\meas$ with measured data products that are invariant to atmospheric inhomogeneity. 
The bispectrum, closure phase, and visibility amplitude data products are invariant to this error, but come at the cost of requiring a non-linear measurement function, $f(\im)$ to \katie{BLAH BLAH express them(?).} 




